A Combinatorial Characterization of Self-Stabilizing Population Protocols

We fully characterize self-stabilizing functions in population protocols for complete interaction graphs. In particular, we investigate self-stabilization in systems of $n$ finite state agents in which a malicious scheduler selects an arbitrary sequence of pairwise interactions under a global fairness condition. We show a necessary and sufficient condition for self-stabilization. Specifically we show that functions without certain set-theoretic conditions are impossible to compute in a self-stabilizing manner. Our main contribution is in the converse, where we construct a self-stabilizing protocol for all other functions that meet this characterization. Our positive construction uses Dickson's Lemma to develop the notion of the root set, a concept that turns out to fundamentally characterize self-stabilization in this model. We believe it may lend to characterizing self-stabilization in more general models as well.

==> extras.tex <==
% TODO: Change increment to change to next root $R_j$. It should be the case that if an agent starts with the wrong root, then eventually it will change roots and reset all agents with input $\sigma$. 


\begin{lemma}
    \label{l:FindAltRoot}
    Let $f: \mathcal{X} \rightarrow Y$ be a function over finite multisets on a finite alphabet, and let $\mathcal{R}$ be a finite and minimally sized root set of $\mathcal{X}$. Let $A \in \mathcal{X}$ be the multiset whose elements are dispersed amongst the agents. $FindAltRoot$ satisfies the following three properties:
    \begin{enumerate}
        \item Each agent takes as input an $i \in \{0, \hdots, |\mathcal{R}| - 1\}$ and an input symbol from $A$.
        \item If an agent has input $i$ such that $f(R_i) \neq f(A)$, then that agent will eventually output 1 forever.
        \item If an agent has input $i$ such that $R_i \subseteq A$, and the current configuration has all agents in some fixed state $q_{init}$, then eventually all agents will output 0 forever.
    \end{enumerate}
\end{lemma}
\begin{proof}
    The first property is immediate. Suppose there is an agent with input $i$ such that $f(R_i) \neq f(A)$. Then since $R_i \not \subseteq A$, by definition of the root set there exists some different root $R_j$ such that $R_j \subseteq A$, which in turn implies $f(R_j) = f(A).$ Note that $MORE_{i,j}$ must be nonempty since otherwise $R_j \subseteq R_i$, which contradicts the minimality of the root set since the root set would be smaller if we excluded $R_i$. For each $\sigma \in MORE_{i,j}$, there will be at least as many agents with input $\sigma$ as there are occurrences in $R_j$, since $R_j \subseteq A$. In particular there will be at least $m_{R_j}(\sigma)$ agents with input $\sigma$. After all these agents interact with each other, it is clear from construction that at least one of the agents will have a $count \geq m_{R_j}(\sigma) - 1$ (note the minus 1 comes from the 0-indexing). This agent will hence have the component corresponding to $\sigma$ in $\varA{HAS-MORE}_{i,j}$ set to a 1. There will be an agent like this for each $\sigma \in MORE_{i,j}$; after having them all interact, they will all bitwise OR their $\varA{HAS-MORE}$ tables which would set $\varA{HAS-MORE}_{i,j}$ to $1^{|MORE_{i,j}|}$ for the last interacting agents. Both of these last agents will now output 1, and since no future bitwise OR's could change $\varA{HAS-MORE}_{i,j}$ they will continue to do so forever. Hence the second property holds.
    
    Suppose that some agent is given input $i$ with $R_i \subseteq A$ (so $f(R_i) = f(A)$) and all agents start in state $q_{init}.$ Suppose that some agent eventually starts outputting 1 because for some $j$, $\varA{HAS-MORE}_{i,j}$ gets set to all 1's (note that the definition states that $MORE_{i,j}$ must be nonempty for this to happen). Since each agent is initialized with 0's in every component of $\varA{HAS-MORE}$, this can only happen if for each $\sigma \in MORE_{i,j}$ there is some agent with $count \geq m_{R_j}(\sigma) - 1$. Because each agent starts with a $0$ count, it then must be the case that there were at least $m_{R_j}(\sigma)$ agents with input symbol $\sigma$ that brought $count$ that high up. We claim that now we have that $R_j \subseteq A$, which we show by considering two cases. If $\sigma \in MORE_{i,j}$, then we already know there are at least $m_{R_j}(\sigma)$ agents with input symbol $\sigma$, so the count of $\sigma$ in $R_j$ is at most the count in $A$. If $\sigma \in \Sigma - MORE_{i,j}$, then the number of occurrences of $\sigma$ in $R_j$ is at most the number in $R_i$, which is at most the number in $A$ since $R_i \subseteq A$. Thus the multiplicity of each element in $R_j$ is at most the respective multiplicity in $A$. Therefore $R_j \subseteq A$ and hence $f(R_i) = f(A) = f(R_j)$. This is a contradiction because $MORE_{i,j}$ would be the empty set. Hence the third property holds.
\end{proof}

% \begin{definition}{$FindAltRoot.$}
%     Let $f: \mathcal{X} \rightarrow Y$ be a function over finite multisets on a finite alphabet, and let $\mathcal{R}$ be a finite and minimally sized root set of $\mathcal{X}$. Define our agent states as $(count, \varA{HAS-MORE})$ where $count$ is a nonnegative integer and $\varA{HAS-MORE}$ is a two index table. The nonnegative integer $count$ is bounded above by the maximum multiplicity occurring in the entire root set. The table $\varA{HAS-MORE}$ is indexed by $i$ and $j$, where each entry is a binary string of length $|MORE_{i,j}|$ (as described in the previous discussion).
%     \begin{align*}
%         &0 \leq counter \leq \max_{R \in \mathcal{R}, \sigma \in \Sigma}m_{R}(\sigma) = M,\\
%         \text{ and } & \varA{HAS-MORE}_{i,j} \in \{0,1\}^{|MORE_{i,j}|}.
%     \end{align*}
%     Each agent is given an input $i \in \{0, \hdots, |\mathcal{R}| - 1\}$ and an input symbol $\sigma$ from some $A \in \mathcal{X}$. Suppose an agent is given input $\sigma \in MORE_{i,j}$ for some $j$ where $f(R_i) \neq f(R_j)$. We want the bit corresponding to $\sigma$ in $\varA{HAS-MORE}_{i,j}$ to be set to 1 if the agent's $count$ is ever at least the number of occurrences of $\sigma$ in $R_j$ (subtracted by 1, since we index by 0). However imposing this requirement on each of the transition rules we design is tedious, since we'd need to explicitly write this in for each rule. To work around this, we add the following extension to all transitions. For any agent with input $(i, \sigma)$ that transitions into state $(count, \varA{HAS-MORE})$, we implicitly bitwise OR the $\varA{HAS-MORE}$ table with an indicator table $INDICATOR$ of same dimension:
%     \begin{align*}
%         INDICATOR_{i,j} = 
%         \begin{cases}
%             1 & \text{ if } count \geq m_{R_j}(\sigma) - 1 \\
%             0 & \text{ otherwise }
%         \end{cases}.
%     \end{align*}
%     Now it is guaranteed (after every agent transitions once) that the corresponding bit will be set if $count$ gets sufficiently high enough.
    
%     Now we describe the state transitions, all of which assume the interacting agents have a common $i$. It is natural to have agents share their $\varA{HAS-MORE}$ tables with each other. Whenever an agent meets another agent, they bitwise OR their $\varA{HAS-MORE}$ tables, which we denote using $\lor$:
%     \begin{gather*}
%         ((*, \varA{HAS-MORE}^1), (i, *)) , ((*, \varA{HAS-MORE}^2), (i, *)) \\ \downarrow \\ ((*, \varA{HAS-MORE}^1 \lor \varA{HAS-MORE}^2), (*, \varA{HAS-MORE}^1 \lor \varA{HAS-MORE}^2))
%     \end{gather*}
    
%     When an agent meets another agent with the same $\sigma$ and same $count$, one of them will increment their $count$ modulo $M$. This guarantees that if there are $m_{R_j}(\sigma)$ agents with symbol $\sigma$ (say, for some root $R_j$ where $f(R_i) \neq f(R_j)$), then one of their $count$ variables will eventually become at least $m_{R_j}(\sigma) - 1$. 
%     \begin{align*}
%         ((count, *), (i, \sigma)) , ((count, *), (i, \sigma)) \rightarrow ((count, *), (count + 1 \mod M, *))
%     \end{align*}
%     Note that these last two transition rules might be invoked simultaneously (which is justifiable since they act upon different components of the state).
    
%     An agent with inputs $i$ and $\sigma$ outputs 1 if there is some $j$ such that $\varA{HAS-MORE}_{i,j} = 1^{|MORE_{i,j}|}$ where $|MORE_{i,j}|$ is nonzero; otherwise the agent outputs 0. Finally we denote $q_{init}$ as the special state where $count = 0$ and $\varA{HAS-MORE}$ is a table of 0's.
% \end{definition}

% \begin{lemma}
%     \label{l:FindAltRoot}
%     Let $f: \mathcal{X} \rightarrow Y$ be a function over finite multisets on a finite alphabet, and let $\mathcal{R}$ be a finite and minimally sized root set of $\mathcal{X}$. Let $A \in \mathcal{X}$ be the multiset whose elements are dispersed amongst the agents. $FindAltRoot$ satisfies the following three properties:
%     \begin{enumerate}
%         \item Each agent in $FindAltRoot$ takes as input an $i \in \{0, \hdots, |\mathcal{R}| - 1\}$ and an input symbol from $A$.
%         \item If all agents are given the same $i$ and $f(R_i) \neq f(A)$, then some agent will eventually output 1 forever.
%         \item If all agents are given the same $i$ and $R_i \subseteq A$ and the current configuration has all agents in some fixed state $q_{init}$, then eventually all agents will output 0 forever.
%     \end{enumerate}
% \end{lemma}
% \begin{proof}
%     The first property is immediate. Suppose all agents are given the same $i$ where $f(R_i) \neq f(A)$. Then since $R_i \not \subseteq A$, by definition of the root set there exists some different root $R_j$ such that $R_j \subseteq A$, which in turn implies $f(R_j) = f(A).$ Note that $MORE_{i,j}$ must be nonempty since otherwise $R_j \subseteq R_i$, which contradicts the minimality of the root set since the root set would be smaller if we excluded $R_i$. For each $\sigma \in MORE_{i,j}$, there will be at least as many agents with input $\sigma$ as there are occurrences in $R_j$, since $R_j \subseteq A$. In particular there will be at least $m_{R_j}(\sigma)$ agents with input $\sigma$. After all these agents interact with each other, it is clear from construction that at least one of the agents will have a $count \geq m_{R_j}(\sigma) - 1$ (note the minus 1 comes from the 0-indexing). This agent will hence have the component corresponding to $\sigma$ in $\varA{HAS-MORE}_{i,j}$ set to a 1. There will be an agent like this for each $\sigma \in MORE_{i,j}$; after having them all interact, they will all bitwise OR their $\varA{HAS-MORE}$ tables which would set $\varA{HAS-MORE}_{i,j}$ to $1^{|MORE_{i,j}|}$ for the last interacting agents. Both of these last agents will now output 1, and since no future bitwise OR's could change $\varA{HAS-MORE}_{i,j}$ they will continue to do so forever. Hence the second property holds.
    
%     Suppose that all agents are given the same $i$ with $R_i \subseteq A$ (so $f(R_i) = f(A)$) and all agents start in state $q_{init}.$ Suppose that some agent eventually starts outputting 1 because for some $j$, $\varA{HAS-MORE}_{i,j}$ gets set to all 1's (note that the definition states that $MORE_{i,j}$ must be nonempty for this to happen). Since each agent is initialized with 0's in every component of $\varA{HAS-MORE}$, this can only happen if for each $\sigma \in MORE_{i,j}$ there is some agent with $count \geq m_{R_j}(\sigma) - 1$. Because each agent starts with a $0$ count, it must be the case that there were at least $m_{R_j}(\sigma)$ agents with input symbol $\sigma$ that brought $count$ that high up. We claim that now we have that $R_j \subseteq A$, which we show by considering two cases. If $\sigma \in MORE_{i,j}$, then we already know there are at least $m_{R_j}(\sigma)$ agents with input symbol $\sigma$, so the count of $\sigma$ in $R_j$ is at most the count in $A$. If $\sigma \in \Sigma - MORE_{i,j}$, then the number of occurrences of $\sigma$ in $R_j$ is at most the number in $R_i$, which is at most the number in $A$ since $R_i \subseteq A$. Thus the multiplicity of each element in $R_j$ is at most the respective multiplicity in $A$. Therefore $R_j \subseteq A$ and hence $f(R_i) = f(A) = f(R_j)$. This is a contradiction because $MORE_{i,j}$ would be the empty set. Hence the third property holds.
% \end{proof}


\section{A Self-Stabilizing Population Protocol}
Now that we have our sub-protocols for (our variant of) the protocol composition, we can construct the overall self-stabilizing protocol. At a high-level, $RootCount$ will select one root in the root set for the agents to output,
\begin{definition}{\textit{The Self-Stabilizing Population Protocol.}}
    Let $f: \mathcal{X} \rightarrow Y$ be a function where $\mathcal{X}$ is a set of finite multisets over a finite alphabet. Let $\mathcal{R}$ be a \textbf{finite} and \textbf{minimally-sized} root set of $\mathcal{X}$. Let $RootCount$ be the modulo-$k$ counter sub-protocol with $k = |\mathcal{R}|$, and let $FindAltRoot$ be our other sub-protocol parameterized by our $f$ and $\mathcal{R}$. Our self-stabilizing population protocol is $RootCount \times FindAltRoot$ with the following notes: \begin{itemize}
        \item If an agent's $RootCount$ is in state $i \in \{0, 1, \hdots, |\mathcal{R}| - 1\}$, the agent outputs $f(R_i)$.
        \item We change the transition function so that every time an agent in $RootCount$ updates its counter, the state corresponding to $FindAltRoot$ gets set to $q_{init}$.
    \end{itemize}
\end{definition}

The following lemma should be clear from the construction of $RootSet$, since conflicting agents override their counter values to come to a consensus.
\begin{lemma}
    \label{L:UniformK-Value}
    Let $\mathcal{C}$ be an execution of the Self-Stabilizing Population Protocol. There exists a configuration $C \in \mathcal{C}$ appearing infinitely often such that all agents have the same counter $\mathrm{i}$ in their agent states for $RootCount$.
\end{lemma}


%%%%% END NEW STUFF


\begin{theorem*}[Self-Stabilizing Population Protocol Theorem]\label{T:SSPP}
    Let $f: \mathcal{X} \rightarrow Y$ be a function computable with population protocols on a complete interaction graph, where $\mathcal{X}$ is a set of multisets. Then
    \begin{align*}
        f \text{ has a self-stabilizing protocol} \iff (\forall A,B \in \mathcal{X}, A \subseteq B \implies f(A) = f(B)).
    \end{align*}
\end{theorem*}
\begin{proof}
    The forward direction was shown previously. We claim the Self-Stabilizing Population Protocol construction for $f$ is a self-stabilizing protocol for $f$. 
    
    Consider an execution of this protocol with input multiset $A$. By Lemma \ref{L:UniformK-Value} there is an infinitely occurring configuration where all agents have the same counter $i$ in $RootCount$. If $f(R_i) \neq f(A)$, then by Property 2 of Lemma \ref{l:FindAltRoot} there eventually will be an agent in $FindAltRoot$ that outputs a 1 forever (``forever'' as in while the counter remains at $i$). Having this agent initiate an interaction with another agent (whose counter is also $i$) will result in both counters being updated to $n = i + 1 \mod |\mathcal{R}|$; then having this agent initiate interactions with every other agent will update all counters to $n$. Moreover, this change in counter will force all of these agents to set their $FindAltRoot$ states to $q_{init}$. In summary the infinitely occurring configuration of all agents having the same counter $i$, $f(R_i) \neq f(A)$, can lead to a configuration where all counters are updated to $i + 1 \mod k$ and $FindAltRoot$ states are all $q_{init}$. By global fairness, this configuration must occur infinitely often as well. This means that the counter will continue iterating until $i$ is such that $f(R_i) = f(A)$. If the counter stopped iterating then the population would successfully converge to $f(R_i) = f(A)$; if not then the counter would continue iterating until $i$ is such that $R_i \subseteq A$ with $q_{init}$ as the $FindAltRoot$ state for all agents. Then by Property 3 of Lemma \ref{l:FindAltRoot} we have that all agents in $FindAltRoot$ will output 0 forever; hence the counter will no longer change so the protocol will converge to $f(R_i) = f(A).$
    
    If Lemma \ref{L:UniformK-Value} yields an infinitely occurring configuration where all agents have the same counter $i$ such that $f(R_i) = f(A)$, then all agents are currently outputting $f(R_i)$. If some agent increments its counter, then having that agent initiate an interaction with every other agent will cause the entire population to have a counter of $i + 1 \mod k$ with $FindAltRoot$ state $q_{init}$. By the previous reasoning this cycling through the root set will eventually make the protocol converge to $f(R_j) = f(A).$
\end{proof}



% MODIFIED VERSION
\begin{definition}{$FindAltRoot.$}
    Let $f: \mathcal{X} \rightarrow Y$ be a function over finite multisets on a finite alphabet, and let $\mathcal{R}$ be a finite and minimally sized root set of $\mathcal{X}$. Define our agent states as $(count, \varA{HAS-MORE})$ where $count$ is a nonnegative integer and $\varA{HAS-MORE}$ is a two index table. The nonnegative integer $count$ is bounded above by the maximum multiplicity occurring in the entire root set, $M$. The table $\varA{HAS-MORE}$ is indexed by $i$ and $j$, where each entry is a binary string of length $|MORE_{i,j}|$ (as described in the previous discussion).
    \begin{align*}
        &0 \leq count \leq M = \max_{R \in \mathcal{R}, \sigma \in \Sigma}m_{R}(\sigma)\\
        \text{ and } & \varA{HAS-MORE}_{i,j} \in \{0,1\}^{|MORE_{i,j}|}.
    \end{align*}
    Each agent is given an input $i \in \{0, \hdots, |\mathcal{R}| - 1\}$ and an input symbol $\sigma$ from some $A \in \mathcal{X}$. Suppose an agent is given input $\sigma \in MORE_{i,j}$ for some $j$ where $f(R_i) \neq f(R_j)$. We want the bit corresponding to $\sigma$ in $\varA{HAS-MORE}_{i,j}$ to be set to 1 if the agent's $count$ is ever at least the number of occurrences of $\sigma$ in $R_j$ (subtracted by 1, since we index by 0). However imposing this requirement on each of the transition rules we design is tedious, since we'd need to explicitly write this in for each rule. To work around this, we add the following extension to all transitions. For any agent with input $(i, \sigma)$ that transitions into state $(count, \varA{HAS-MORE})$, we implicitly bitwise OR the $\varA{HAS-MORE}$ table with an indicator table $INDICATOR$ of same dimension:
    \begin{align*}
        INDICATOR_{i,j} = 
        \begin{cases}
            1 & \text{ if } count \geq m_{R_j}(\sigma) - 1 \\
            0 & \text{ otherwise }
        \end{cases}.
    \end{align*}
    Now it is guaranteed (after every agent transitions once) that the corresponding bit will be set if $count$ gets sufficiently high enough.
    
    Now we describe the state transitions. It is natural to have agents share their $\varA{HAS-MORE}$ tables with each other to share their collected information about the population. Whenever an agent meets another agent, they bitwise OR their $\varA{HAS-MORE}$ tables, which we denote using $\lor$:
    \begin{gather*}
        ((*, \varA{HAS-MORE}^1), (*, *)) , ((*, \varA{HAS-MORE}^2), (*, *)) \\ \downarrow \\ ((*, \varA{HAS-MORE}^1 \lor \varA{HAS-MORE}^2), (*, \varA{HAS-MORE}^1 \lor \varA{HAS-MORE}^2))
    \end{gather*}
    
    When an agent meets another agent with the same $\sigma$ and same $count$, one of them will increment their $count$ modulo $M$. This guarantees that if there are $m_{R_j}(\sigma)$ agents with symbol $\sigma$ (say, for some root $R_j$ where $f(R_i) \neq f(R_j)$), then one of their $count$ variables will eventually become at least $m_{R_j}(\sigma) - 1$. 
    \begin{align*}
        ((count, *), (*, \sigma)) , ((count, *), (*, \sigma)) \rightarrow ((count, *), (count + 1 \mod M, *))
    \end{align*}
    Note that these last two transition rules might be invoked simultaneously (which is justifiable since they act upon different components of the state).
    
    An agent with inputs $i$ and $\sigma$ outputs 1 if there is some $j$ such that $\varA{HAS-MORE}_{i,j} = 1^{|MORE_{i,j}|}$ where $|MORE_{i,j}|$ is nonzero; otherwise the agent outputs 0. Finally we denote $q_{init}$ as the special state where $count = 0$ and $\varA{HAS-MORE}$ is a table of 0's.
\end{definition}


\iffalse
To do this, each agent state will include an index $root$, and the first thing the population will come to a consensus on is a common value for $root$. That $root$ determines each individual agent's output; if $R$ is the root in the root set corresponding to index $root$, then an agent will output $f(R)$. Once everyone has agreed on a $root$, the population will be effectively ``guessing'' that $R \subseteq A$. To make progress, they need a way to determine if their output is wrong (perhaps $f(R) = f(A)$ even though $R \not \subseteq A$, but the output is right so we don't care).

To have the population determine that $f(R)$ is actually \textit{not} the right output, we can program the protocol to move on to $root + 1$ when some impossible condition is observed that indicates $f(R) \neq f(A)$. One such impossible condition occurs if there is another root with a \textit{different} output under $f$ that is \textit{also} a subset to the population. This would demonstrate that $f(R) \neq f(A)$ since the subgraph property says that the other root outputs the correct answer under $f$! 

To formalize this, let $A$ be the population's input. Suppose the population has incorrectly agreed upon a root $Wrong \in \mathcal{R}$ such that $f(Wrong) \neq f(A)$; so all agents are wrongly outputting $f(Wrong)$. Let $Right$ be another root in $\mathcal{R}$ such that $f(Right) \neq f(Wrong)$ (the choice in name $Right$ will become clear). Consider the set $\varA{MORE-NEQ}$ defined earlier, where we are looking at the symbols appearing strictly more often in $Right$ than in $Wrong$ (and note that $\varA{MORE-NEQ} = MORE$ since $f(Wrong) \neq f(Right)$). Suppose that we observe that for any symbol $\sigma \in \varA{MORE-NEQ}$ there are at least as many agents in the population with input $\sigma$ as there are occurrences of $\sigma$ in $Right$. Using the multiplicity notation, we might denote this property as 

\begin{center}
    For any $\sigma \in \varA{MORE-NEQ}$, the population has at least $m_{Right}(\sigma)$ agents with input $\sigma$. \hspace{1em} $(*)$\\
\end{center}

\noindent The population's hypothesis that $Wrong \subseteq A$ is then wrong. Suppose $Wrong \subseteq A$. We've just observed that the symbols occurring strictly more often in $Right$ than in $Wrong$ have at least the same number of agents with that input. Furthermore the other symbols (i.e. symbols in $\Sigma - \varA{MORE-NEQ}$) have multiplicity less than or equal to the corresponding multiplicity in $Wrong$, and hence have multiplicity less than or equal to the corresponding multiplicity in $A$ since $Wrong \subseteq A$ by assumption. This means that $Right \subseteq A$ and hence $f(Right) = f(A)$. This is a contradiction because $f(Wrong) \neq f(Right) = f(A)$, implying $Wrong \not \subseteq f(A)$.

So observing condition $(*)$ in the population indicates that the chosen root is actually not a subset to the population (and by contrapositive, if the root is a subset, $(*)$ wouldn't be observed). Conversely, if the selected root $Wrong \not \subseteq A$, then then there exists some correct root $Right \subseteq A$; then the condition $(*)$ holds trivially because there have to be at least as many agents with any input $\sigma$, as $Right$ holds a subset of the population's inputs. Hence $(*)$ can be detected if and only if the population's selected root is outputting the wrong answer. This gives us a condition to look for in our protocol; if we program the protocol so that it has to \textit{eventually} determine if this condition is true, then we can program it to increment $root$. Hence the population would eventually self-stabilize to the appropriate root, $Right$.

This outlines the argument at a high level. We now dive into the protocol itself.
\fi

Some final definitions are needed for the protocol we define in Section \ref{SS:Protocol}. Let $S$ and $T$ be finite multisets on an alphabet $\Sigma$. Define \textit{MORE} as the set of alphabet symbols that occur strictly more frequently in $S$ than in $T$. If we denote the multiplicity (number of occurrences) of alphabet symbol $\sigma \in \Sigma$ within a finite multiset $X$ as $m_X(\sigma)$, we can more formally describe this set as follows: $$\text{\textit{MORE}} = \{\sigma \in \Sigma \mid m_S(\sigma) > m_T(\sigma) \}.$$ In the context of a function $f: \mathcal{X} \rightarrow Y$ satisfying the subgraph property and two sets $S, T \in \mathcal{X}$, we will find it useful to define the same set except with the extra condition that the set is empty if $f(S) = f(T)$. For this reason we will refer to the set as $\varA{MORE-NEQ}$, in that we want the alphabet symbols that occur \textit{more} often in $S$ when $f(S)$ is \textit{not equal} to $f(T)$:
\begin{align*}
    \varA{MORE-NEQ} &=
        \begin{cases}
            \text{\textit{MORE}} & \text{if } f(S) \neq f(T) \\
            \emptyset & \text{otherwise}
        \end{cases}.
\end{align*}
Note that in the way that these were defined, $S$ and $T$ were clear from context because they were explicitly mentioned. We will maintain this convention of explicitly mentioning the sets being compared in $\varA{MORE-NEQ}$ before using it.

\section{The Self-Stabilizing Population Protocol}
\subsection{Proof of Lemma \ref{L:InputSymbols}} \label{A:InputSymbols}

% input field becomes reflective of agent input
\begin{lemma}
    Let $\mathcal{C}$ be an execution of the Self-Stabilizing Population Protocol. After a finite number of configurations, all configurations afterwards have all agents with input $\sigma \in \Sigma$ in a state of the form $(\sigma, *, *, *, \hdots, *)$.
\end{lemma}
\begin{proof}
    This is evident from transition rule $(1a)$. If any agent with input $\sigma$ has its state field $input$ with $input \neq \sigma$, a single interaction will change $input$ to $\sigma$. All other transition rules assume this property holds for the agent, so this agent will always have $input = \sigma$. Clearly this property holds after a finite number of interactions (specifically after each agent has initiated an interaction).
\end{proof}


\subsection{Proof of Lemma \ref{L:UniformK-Value}} \label{A:UniformK-Value}

% Uniform value for root occurs infinitely often
\begin{lemma*}
    Let $\mathcal{C}$ be an execution of the Self-Stabilizing Population Protocol. There exists a configuration $C \in \mathcal{C}$ appearing infinitely often such that all agents have the same index $\mathrm{root}$ in their agent states.
\end{lemma*}
\begin{proof}
    Since there are a finite number of configurations, there must be some configuration $C' \in \mathcal{C}$ that occurs infinitely often. By Lemma \ref{L:InputSymbols}, it must be the case that every agent's $input$ field reflects the agent's actual input symbol. Select any agent with highest value for $root$ in the population, which we call $root_{max}$. If $root_{max} = 0$ then we are done. Otherwise have this agent initiate an interaction with all other agents in the population whose $root$ value is such that $0 < root < root_{max}$. Since $root \neq 0$, transition rule $(1b)$ enforces that the other agents must change their value for $root$ to $root_{max}$. 
    
    If there are no agents with $root = 0$, we are done. Otherwise we have just $root_{max}$ agents and $root = 0$ agents. Have the $root_{max}$ agents initiate an interaction with agents with $root = 0$. If $root_{max} = |\mathcal{R}| - 1$, transition rule $(1c)$ will force all agents to have $root = |\mathcal{R}| - 1$. If $root_{max} \neq |\mathcal{R}| - 1$, transition rule $(1b)$ will also force all agents to take on a $root$ value of $root_{max}$. The resultant configuration, $C$, has all agents with the same value for $root$ (specifically $root_{max}$). Since $C' \xrightarrow{*} C$, and $C'$ appears infinitely often, $C$ must also appear infinitely often by global fairness.
\end{proof}

\subsection{Proof of Lemma \ref{L:InfiniteCorrectOutput}} \label{A:InfiniteCorrectOutput}
\begin{lemma*}
    Let $\mathcal{C}$ be an execution of the Self-Stabilizing Population Protocol, let $R$ be the root corresponding to $\mathrm{root}$, and let the input to the population be $A$. There exists an infinitely occurring configuration $C \in \mathcal{C}$ such that all agents have the same $\mathrm{root}$ and $f(R) = f(A)$.
\end{lemma*}
\begin{proof}
    Let $C' \in \mathcal{C}$ be the configuration from Lemma \ref{L:UniformK-Value}. Now suppose $f(R) \neq f(A)$, which implies $R \not \subseteq A$. By definition of root set, there exists a $Right \in \mathcal{R}$ such that $Right \subseteq A$, and thus $f(Right) = f(A) \neq f(R)$. Let $S = Right$ and $T = R$; define $\varA{MORE-NEQ}$ as before: since $f(S) \neq f(T)$, it is the set of symbols occuring strictly more often in $S$ than in $T$. The set $\varA{MORE-NEQ}$ is nonempty; if it was empty then $Right \subseteq R$, contradicting the minimality of the root set (i.e. $\mathcal{R} - \{R\}$ would be a smaller root set).
    
    Let $\sigma \in \varA{MORE-NEQ}$. By definition of $\varA{MORE-NEQ}$ this means that $m_{R}(\sigma) < m_{Right}(\sigma)$, and since $Right \subseteq A$ we have that
    \begin{align*}
        m_{R}(\sigma) < m_{Right}(\sigma) \leq m_A(\sigma).
    \end{align*}
    We claim that there must eventually be an agent with $count \geq m_{Right}(\sigma) - 1$. If not, then all $m_A(\sigma)$ agents with input symbol $\sigma$ must have their $count$ such that $0 \leq count \leq m_{R_n}(a) - 2$. Additionally the interaction of two agents with the same $input, count,$ and $root$ will yield (via transition rule (1f)) resultant component $count$ values of $count$ and $count + 1$ respectively. Global fairness allows us to then deduce that all agents with input $\sigma$ have different values for $count$. There are $m_{Right}(\sigma) - 1$ different values, and $m_A(\sigma)$ agents.  As $m_A(\sigma) \geq m_{Right}(\sigma) > m_{Right}(\sigma) - 1$ agents, by the Pigeonhole Principle there must then be at least two agents with the same $count$, a contradiction. 
    
    Thus for all $\sigma \in \varA{MORE-NEQ}$ there is an agent with $count \geq m_{Right}(\sigma) - 1$. Furthermore notice that we have $\sigma \in \varA{MORE-NEQ}$ and $count \geq m_{Right}(\sigma) - 1$. Let $i$ be the index of $\sigma$ in the total ordering of $\varA{MORE-NEQ}$; then we have for this agent that the $i^{th}$ symbol of $\textbf{symbols}_n$ is set to a 1 (recall the definition of $\vec{\varphi}$ from the protocol definition that assures that this condition holds). Now we can have each of these $|\varA{MORE-NEQ}|$ agents with their set bit in $\textbf{symbols}_n$ interact with each other to bitwise OR their vectors, thereby making a full vector of 1's. Formally, we will have by transition rule $(1e)$
    \begin{align*}
        \textbf{sybmols}_n = \bigvee_{\sigma \in \varA{MORE-NEQ}} \hat{e}_{i} = 1^{|\varA{MORE-NEQ}|},
    \end{align*}
    where $i$ corresponds to the index of $\sigma$ and $\hat{e}_i$ is the unit vector in the $i^{th}$ component. Transition rule $(1e)$ specifies that once $\textbf{symbols}_n = 1^{|\varA{MORE-NEQ}|}$, the value of $root$ for the agent increases to $root + 1 \mod |\mathcal{R}|$. Having this agent interact with all agents in the population using transition rule
    \begin{itemize}
        \item $(1b)$, if at least one of $root$ and $root+1$ is neither $|\mathcal{R}| - 1$ nor 0
        \item $(1c)$, if $root + 1 = |\mathcal{R}| - 1$ and $root = 0$
        \item or $(1d)$, if $root + 1 = 0$ and $root = |\mathcal{R}| - 1$
    \end{itemize}
    will cause the entire population to have a $root$ value of $root + 1 \mod |\mathcal{R}|$.
    
    Now we have shown that if $C$ is an infinitely appearing configuration where all agents have the same $root$ where $f(R) \neq f(A)$, then $C'$ is an infinitely appearing configuration where all agents have the same incremented $root$ value of $root + 1$. This rule can be applied repeatedly to cycle through the values of $root \in \{0, \hdots, |\mathcal{R}| - 1\}$ until we reach a value of $root$ such that $f(R) = f(A)$. Thus that configuration must be infinitely occurring as well.
\end{proof}
\begin{corollary*}
    Let $\mathcal{C}$ be an execution of the Self-Stabilizing Population Protocol. If $C \in \mathcal{C}$ is an infinitely occurring configuration where all agents have the same $\mathrm{root}$ where $f(R) \neq f(A)$, then $C'$ is an infinitely occurring configuration in $\mathcal{C}$ where all agents have the same incremented index value of $\mathrm{root} + 1$.
\end{corollary*}

\subsection{Proof of Main Theorem} \label{A:SS-PP}
\begin{theorem*}[Self-Stabilizing Population Protocol Theorem] 
    Let $f: \mathcal{X} \rightarrow Y$ be a function computable with population protocols on a complete interaction graph, where $\mathcal{X}$ is a set of multisets. Then
    \begin{align*}
        f \text{ has a self-stabilizing protocol} \iff (\forall A,B \in \mathcal{X}, A \subseteq B \implies f(A) = f(B)).
    \end{align*}
\end{theorem*}
\begin{proof}
    The forward direction is shown in Theorem \ref{T:Subgraph}. We continue the proof of the converse.
    
    Suppose that the Self-Stabilizing Population Protocol does not converge in some execution $\mathcal{C}$. Let $C \in \mathcal{C}$ be the infinitely occurring configuration with uniform value of $root$ from Lemma \ref{L:UniformK-Value}. Let $R$ be the root in the root set corresponding to index $root$. If the current $root$ is such that $f(R) \neq f(A)$, then by Corollary \ref{C:CycleProperty} the population will move to the next value of $root + 1$. If the $root$ is such that $f(R) = f(A)$, then since we do not converge it must be that transition rule $(1e)$ eventually moves two members to $root + 1$ (since it is the only rule that can result in a change in output). Having these members initiate interaction with everyone using transition rule
    \begin{itemize}
        \item $(1b)$, if at least one of $root$ and $root+1$ is neither $|\mathcal{R}| - 1$ nor 0
        \item $(1c)$, if $root + 1 = |\mathcal{R}| - 1$ and $root = 0$
        \item or $(1d)$, if $root + 1 = 0$ and $root = |\mathcal{R}| - 1$
    \end{itemize}
    causes the entire population to increment their $root$. Thus for all $root \in \{0, \hdots, |\mathcal{R}| - 1\}$, there is an infinitely occurring configuration in which all agents have the same $root$.
    
    By definition of the root set, there exists a $Right \in \mathcal{R}$ such that $Right \subseteq A$ and thus $f(Right) = f(A)$. Let $n$ be the index corresponding to $Right \in \mathcal{R}$. Let $C''$ be the infinitely occurring configuration in which the population is shifting from $root$ value of $n - 1 \mod |\mathcal{R}|$ to $n$; in other words, when the first two agents of $root = n$ emerge in the population full of agents with $root = n - 1$. Have \textit{one} of the agents \textit{initiate} an interaction with every agent with $root = n - 1$; by transition rule $(1b), (1c)$ or $(1d)$ the entire population will have $root = n$, and every agent with input $\sigma$ will have state component $count = 0$. Furthermore, the bit vectors are all $\textbf{symbols}_m = \vec{\varphi}$ (recall that every vector is bitwise OR'd with $\vec{\varphi}$ upon a transition). Now for any two agents with the same $input$ and $count$, having them interact will cause one's $count$ to increase by 1 via transition rule $(1f)$; since the agent component states start at $count = 0$, the highest $count$ an agent with input $\sigma$ can have satisfies $count \leq m_A(\sigma) - 1$.
    
    Since the population now has to shift to $n + 1 \mod |\mathcal{R}|$, there must be some $Wrong \in \mathcal{R}$ whose corresponding bit vector becomes all 1's. Consider $\varA{MORE-NEQ}$ with $S = Wrong$ and $T = Right$; since a shift occurs due to $Wrong$'s bit vector, it must be that $\varA{MORE-NEQ}$ is nonempty. For all $\sigma \in \varA{MORE-NEQ}$ there eventually will be an agent with state value $input = \sigma$ and $count \geq m_{Wrong}(\sigma) - 1$, since this is the only way to invoke the second case of transition rule $(1e)$. Since for all $\sigma \in \varA{MORE-NEQ}$ we have $m_{Wrong}(\sigma) - 1 \leq count \leq m_A(\sigma) - 1$, we have that $m_{Wrong}(\sigma) \leq m_A(\sigma)$. By definition of $\varA{MORE-NEQ}$ we also know that $m_{Right}(\sigma) < m_{Wrong}(\sigma) \leq m_A(\sigma)$; for $\sigma' \in \Sigma - \varA{MORE-NEQ}$ (which are the symbols that occur in $Right$ at least as often as in $Wrong$) we also have that $m_{Wrong}(\sigma') \leq m_{Right}(\sigma') \leq m_A(\sigma')$, where the last inequality is because $Right \subseteq A$. Therefore for all $x \in \Sigma, m_{Wrong}(x) \leq m_A(x)$ and thus $Wrong \subseteq A \implies f(Wrong) = f(A)$. However this contradicts the fact that $\varA{MORE-NEQ}$ is nonempty, since $f(Wrong) = f(A) = f(Right) \implies \varA{MORE-NEQ} = \emptyset$. This is a contradiction, and thus the protocol must converge.
\end{proof}


\iffalse
\begin{definition}{\textit{The Self-Stabilizing Population Protocol.}}
    We formally specify a self-stabilizing protocol. Let $f: \mathcal{X} \rightarrow Y$ be a function computable with population protocols with the additional property that
    \begin{align*}
        \forall A, B \in \mathcal{X}, A \subseteq B \implies f(A) = f(B).
    \end{align*}
    
    Let $\mathcal{R} \subseteq \mathcal{X}$ be a \textbf{finite} and \textbf{minimally sized} root set of $\mathcal{X}$ with a fixed total ordering. We define an agent state as a tuple of the form $$(input, count, root, \textbf{symbols}_0, \hdots, \textbf{symbols}_{|\mathcal{R}| - 1})$$ as follows:
    \begin{itemize}
        \item $input$ is the agent's input symbol. Agents may be started in an arbitrary state, so this entry may not be the agent's input symbol at first. However we can enforce that every agent will update $input$ to be its own input symbol after a single transition. See transition rule (1a).
        \item $count$ is used as a means of ``counting''. Specifically, $count$ is an upper-bounded, nonnegative integer used to count agents with input symbol $input$ modulo the maximum multiplicity of $input$ in the root set $\mathcal{R}$. More formally,
        \begin{align*}
            0 \leq count \leq \left ( \max_{R \in \mathcal{R}} m_R(input) \right) - 1
        \end{align*}
        If two agents with identical $count$ meet, one will increment $count$ (modulo our upper bound).
        \item $root$ is an index into our totally ordered root set $\mathcal{R}:$
        \begin{align*}
            root \in \{0, 1, \hdots, |\mathcal{R}| - 1\}.
        \end{align*}
        The root $R \in \mathcal{R}$ corresponding to $root$ is the root being tested as subset of the population, as described earlier in this section. An agent's output is $f(R)$, and each agent in the population will uniformly iterate through values of $root$ until the correct output is determined.
        \item $\textbf{symbols}_n$ is as follows. Suppose the agent is in state $(input, count, root, \textbf{symbols}_0, \hdots,$  $\textbf{symbols}_{|\mathcal{R}|-1})$. Let $T$ be the root corresponding to $root$, and similarly let $S$ be the $n^{th}$ root. Let $MORE$ be defined as described earlier: the set of symbols occurring strictly more often in $S$ than in $T$. Let $\varA{MORE-NEQ}$ also be defined as described earlier: it is $MORE$ when $f(S) \neq f(T)$ and the empty set otherwise. Fix a total ordering on $\varA{MORE-NEQ}$.
        
        $\textbf{symbols}_n$ is then a binary vector of length $|\varA{MORE-NEQ}|$; note that we admit the possibility of the vector having no elements. This part of the agent states is critical to determining if $(*)$ becomes satisfied. The $i^{th}$ bit is set to 1 when the $i^{th}$ symbol in $\varA{MORE-NEQ}$ occurs in the population at least as many times as it does in $S$ (rather, it is set to 1 once the population counts enough agents with that symbol). Otherwise the bit is set to 0. Once all the bits are 1, condition $(*)$ is satisfied, and the population increments $root$ modulo its largest value.
        
        \iffalse
        {
        If the agent's symbol $i$ is in $B_{n,k}$, then $B_{n,k}$ is nonempty, so the conditions $f(R_n) \neq f(R_k)$ and $m_{R_n}(i) > m_{R_k}(i)$ are satisfied. Additionally, $j \geq m_{R_n}(i) - 1$ implies there are at least $m_{R_n}(i)$ agents\footnote{In reality agents can start in any arbitrary state, so the existence of an agent with a $j$ satisfying this condition does not immediately imply that there are $m_{R_n}(i)$ agents with input $i$. However our protocol will be designed so that eventually this will be the case, so this intuition is eventually valid.} with input $i$. Thus the rule we use is that if an agent is in state $(q_i^j, k, \vec{r}_0, \hdots, \vec{r}_n, \hdots, \vec{r}_{|\mathcal{R}| - 1})$ with input $i \in B_{n,k}$ and $j \geq m_{R_n}(i) - 1$, the component in $\vec{r}_n$ corresponding to $i$ will be set\footnote{Note that each $i \in B_{n,k}$ will each have their own component in $\vec{r}_n$. If $B_{n,k}$ is the empty set (because $f(R_n) = f(R_k)$) this is vacuously true; otherwise $B_{n,k} = C_{n,k}$, and the dimension of $\vec{r}_n$ is exactly $|C_{n,k}|$.} to a 1. Notice that if the bit vector gets set to all 1's, then the condition $(*)$ is satisfied; our transition rule (2e) will increment the $k$-value in this case.
        
        We describe this more formally. Suppose an agent is in state $(q_i^j, k, \vec{r}_0, \hdots, \vec{r}_n, \hdots, \vec{r}_{|\mathcal{R}| - 1})$. Define $\hat{e}_{l}$ as a unit vector in the $l^{th}$ component, where $\hat{e}_{l}$ (like $\vec{r}_n$) has dimension $|C_{n,k}|$. Then we impose the following property on $\vec{r}_n$:
        \begin{gather}
            i \in B_{n,k} \text{ and } j \geq m_{R_n}(i) - 1 \implies \vec{r}_n \cdot \hat{e}_{\tau^{-1}_{n,k}(i)} = 1.
        \end{gather}
        This just sets the vector component of $\vec{r}_n$ corresponding to $i \in B_{n,k}$ to a 1 when the described conditions hold. To maintain (1), any transition for an agent resulting in state $(q_i^j, k, \vec{r}_0, \hdots, \vec{r}_{|\mathcal{R}| - 1})$ will have the vector $\vec{r}_n$ bitwise OR'd with vector
        \begin{align*}
            \vec{\varphi}_{i,j,k,n} = 
            \begin{cases}
                \hat{e}_{\tau^{-1}_{n,k}(i)} & \text{if } i \in B_{n,k} \text{ and } j \geq m_{R_n} - 1 \\
                \vec{0} & \text{otherwise}
            \end{cases}.
        \end{align*}
        Though $\vec{\varphi}_{i,j,k,n}$ will be bitwise OR'd with the agent's vector $\vec{r}_n$, we will omit it from our transition descriptions for the sake of brevity.
        }
        \fi
        
    \end{itemize}
    
    \begin{subequations}
    We will now begin our state transition definition. First, however, we address an implicit transition that we omit for brevity, but that exists in all of our transitions nonetheless. Suppose that there is an agent in state $(input, count, root, \textbf{symbols}_0, \hdots, \textbf{symbols}_{|\mathcal{R}| - 1})$. Let $S$ be the $n^{th}$ root and let $T$ be the root corresponding to $root$. Consider the set $\varA{MORE-NEQ}$ in this context (with $S$ and $T$ used in the usual way). As described in the section about $\textbf{symbols}_n$, we want the $i^{th}$ bit to be 1 when the $i^{th}$ symbol in $\varA{MORE-NEQ}$ occurs in the population at least as many times as it does in $S$. As we will be using the $count$ field for ``counting,'' we will want to ensure that if $count$ is greater than or equal to the multiplicity of $input$ in $S$, then the corresponding bit in $\textbf{symbols}_n$ will be set to a 1. More formally, if $input$ is the $i^{th}$ symbol of $\varA{MORE-NEQ}$, we want that $$count \geq m_S(input) \implies i^{th} \text{ bit of } \textbf{symbols}_n \text{ is a 1}.$$ This requirement should allude to how the protocol is trying to behave in general. Every agent with symbol $input$ will meet other agents with symbol $input$, and their meeting results in one of them incrementing their $count$. Eventually if someone's $count$ is large enough, then we know that the bit corresponding to $input$ should be set to a 1; and if one bit vector is set to all 1's, the condition $(*)$ is satisfied\footnote{This description doesn't seem self-stabilizing, but that's only because this is the high-level intuition. In reality even if an agent is initialized with a nonzero $count$, the presence of enough agents with the same $input$ will drive \textbf{someone's} $count$ to exceed our threshold. We will formalize this via the Pigeonhole Principle.}. This will be explained more formally in the proof of correctness afterwards. 
    
    Maintaining the previous implication isn't too difficult. Consider an agent transitioning into a state of the form $(input, count, root, \textbf{symbols}_0, \hdots, \textbf{symbols}_{|\mathcal{R}| - 1})$. If $input \in \varA{MORE-NEQ}$ (with $S$ still the $n^{th}$ root and $T$ still the root corresponding to $root$), call its index $i$. Let $\hat{e}_i$ be a unit vector in the $i^{th}$ component of dimension $|\varA{MORE-NEQ}|$. Then $\textbf{symbols}_n$ is bitwise OR'd the following vector so that the implication always holds:
    \begin{align*}
        \vec{\varphi} = 
        \begin{cases}
            \hat{e}_i & \text{if } input \in \varA{MORE-NEQ} \text{ and } count \geq m_S(input) \\
            0 & otherwise
        \end{cases}.
    \end{align*}
    
    Now we move to our actual transitions. Note that a $*$ denotes a wildcard, and we will denote $\delta((q_1,x_1), (q_2,x_2)) = (q'_1, q'_2)$ as $$(q_1,x_1), (q_2,x_2) \rightarrow q'_1, q'_2.$$ Our first transition just guarantees that eventually any agent with input $\sigma$ will have a $input = \sigma$. Note we could do without this rule since the transition functions depend on both agents' state \textit{and} input; however $input$ is convenient notation.
    \begin{gather}
        % TRANSITION RULE 1
        ((input, count, *, *, \hdots, *), \sigma),      % Initiator starting state 
        ((*, *, *, \hdots, *),*)                        % Responder starting state  
        \rightarrow 
        (\sigma, 0, *, *, \hdots, *),                   % Initiator transition state
        (*, *, *, \hdots, *) \\                         % Responder transition state
        \text{where } input \neq \sigma\notag.
    \end{gather}
    The second transition rule will be used to have the population come to a consensus on a common value for $root$. It asserts that if two agents have conflicting values for $root$, they will both resolve to the larger value when the two values are not both 0 and $|\mathcal{R}| - 1$. We exclude these because we want to be able to ``loop'' from $root = |\mathcal{R}| - 1$ to $root = 0$.
    \begin{gather}
        % TRANSITION RULE 2
        ((\sigma_1, count_1, root_1, *, \hdots, *), \sigma_1),                                                          % Initiator Starting State
        ((\sigma_2, count_2, root_2, \textbf{symbols}_0, \hdots, \textbf{symbols}_{|\mathcal{R}|-1}), \sigma_2) \\      % Responder Starting State
        \rightarrow 
        (\sigma_1, 0, root_2, \textbf{symbols}_0, \hdots, \textbf{symbols}_{|\mathcal{R}|-1}),                          % Initiator Transition State
        (\sigma_2, count_2, root_2, \textbf{symbols}_0, \hdots, \textbf{symbols}_{|\mathcal{R}|-1}) \notag \\           % Responder Transition State
        %
        \text{where } root_2 > root_1 \text{ and } (root_2 \neq |\mathcal{R}| - 1 \text{ or } root_1 \neq 0). \notag
    \end{gather}
    The third and fourth transition rules say that if those values are both 0 and $|\mathcal{R}| - 1$ then both agents resolve to the initiator's $root$.
    \begin{gather}
        % TRANSITION RULE 3
        ((\sigma_1, count_1, |\mathcal{R}| - 1, *, \hdots, *), \sigma_1),                                                       % Initiator Starting State
        ((\sigma_2, count_2, 0, \textbf{symbols}_0, \hdots, \textbf{symbols}_{|\mathcal{R}|-1}), \sigma_2) \\                   % Responder Starting State
        \rightarrow 
        (\sigma_1, 0, |\mathcal{R}| - 1, \textbf{symbols}_0, \hdots, \textbf{symbols}_{|\mathcal{R}|-1}),                       % Initiator Transition State
        (\sigma_2, count_2, |\mathcal{R}| - 1, \textbf{symbols}_0, \hdots, \textbf{symbols}_{|\mathcal{R}|-1}) \notag \\        % Responder Transition State
        % TRANSITION RULE 4
        ((\sigma_1, count_1, 0, *, \hdots, *), \sigma_1),                                                                       % Initiator Starting State
        ((\sigma_2, count_2, |\mathcal{R}| - 1, \textbf{symbols}_0, \hdots, \textbf{symbols}_{|\mathcal{R}|-1}), \sigma_2) \\   % Responder Transition State
        \rightarrow 
        (\sigma_1, 0, 0, \textbf{symbols}_0, \hdots, \textbf{symbols}_{|\mathcal{R}|-1}),                                       % Initiator Starting State 
        (\sigma_2, count_2, 0, \textbf{symbols}_0, \hdots, \textbf{symbols}_{|\mathcal{R}|-1}) \notag                           % Responder Transition State
    \end{gather}
    Notice that $(1b), (1c)$ and $(1d)$ in tandem guarantee that eventually the entire population will adopt a singular value for $root$. Now take $\textbf{r} \lor \textbf{s}$ as a bitwise OR of two bit vectors. The fifth transition rule says that two agents with the same value for $root$ (and with different values for $count$) will bitwise OR each of their vectors $\textbf{symbols}_m \lor \textbf{symbols}'_m$ for all $m$; if this results in a vector of all 1's, the agents reset to the form $(input, 0, root + 1, \textbf{0}, \hdots, \textbf{0})$, where addition is taking modulo $|\mathcal{R}|$. We will show that then eventually, if $(*)$ is satisfied, an agent will have some $\textbf{symbols}_n$ become a bit string of all 1's, causing the population to increment the $root$.
    \begin{gather}
        % TRANSITION RULE 5
        ((\sigma_1, count_1, root, \textbf{symbols}_0, \hdots, \textbf{symbols}_{|\mathcal{R}|-1}),\sigma_1), \notag \\                   % Initiator Starting State
        ((\sigma_2, count_2, root, \textbf{symbols}'_0, \hdots, \textbf{symbols}'_{|\mathcal{R}|-1}),\sigma_2) \notag \\        % Responder Starting State
        \rightarrow 
        \begin{cases}
            (\sigma_1, 0, root + 1, \textbf{0}, \hdots, \textbf{0}),                                                            % Initiator Transition State (if 1 vector)
            (\sigma_2, 0, root + 1, \textbf{0}, \hdots, \textbf{0})                                                             % Responder Transition State (if 1 vector)
                    & \hspace{-10em} \text{if } \exists n, \textbf{symbols}_n \lor \textbf{symbols}'_n = \textbf{1}, \\ & \hspace{-10em}\text{both }\textbf{symbols}_n \text{ and } \textbf{symbols}'_n \\ & \hspace{-10em} \text{nonempty }\\
            \\
            (\sigma_1, count_1, root, \textbf{symbols}_0 \lor \textbf{symbols}'_0, \hdots,                                      % Initiator Transition State (otherwise)
                \textbf{symbols}_{|\mathcal{R}| - 1} \lor \textbf{symbols}'_{|\mathcal{R}|-1}), \\                              
            (\sigma_2, count_2, root, \textbf{symbols}_0 \lor  \textbf{symbols}'_0, \hdots,                                      % Responder Transition State (otherwise)
                \textbf{symbols}_{|\mathcal{R}| - 1} \lor \textbf{symbols}'_{|\mathcal{R}|-1}) 
                    & \text{otherwise}
        \end{cases} \\
        \text{where } count_1 \neq count_2 \notag
    \end{gather}
    The last transition rule states that two agents with the same values for $input$, $count$, and $root$ have the responder increment its $count$, addition taken modulo $\left ( \max_{R \in \mathcal{R}} m_R(input)  \right )$.
    \begin{gather}
        % TRANSITION RULE 6
        ((input, count, root, *, \hdots, *),input),                 % Initiator Starting State
        ((input, count, root, *, \hdots, *), input) \\ \notag       % Responder Starting State
        \rightarrow 
        ((input, count, root, *, \hdots, *),                        % Initiator Transition State
        (input, count + 1, root, *, \hdots, *))                     % Responder Transition State
    \end{gather}
    
    \end{subequations}
    \hline
\end{definition}

Execution should generally be like so. We start our population in any arbitrary configuration. Agents begin meeting, conflicting values of $root$ are reconciled, and eventually every agent has an identical value for $root$. Let $R$ be the root corresponding to $root$, and let $A$ be the input to the population. We then show that if $f(R) \neq f(A)$, the entire population will increment their $root$ index to $root + 1 \mod |\mathcal{R}|$. We also show that we can converge if $root$ is such that $R \subseteq A$; this can be used to argue that the population would have to converge to $f(A)$. We will do this through a sequence of lemmas showing that in any execution $\mathcal{C}$ of the Self-Stabilizing Population Protocol, some desirable configuration $C$ occurs infinitely often. The final proof will show that the infinitely occurring configuration where all agents are outputting the correct answer never has an agent change output, demonstrating convergence.

The following lemma is a simple application of transition rule $(1a)$. See Appendix \ref{A:InputSymbols}.
\begin{lemma}
    \label{L:InputSymbols}
    Let $\mathcal{C}$ be an execution of the Self-Stabilizing Population Protocol. After a finite number of configurations, all configurations afterwards have all agents with input $\sigma \in \Sigma$ in a state of the form $(\sigma, *, *, *, \hdots, *)$.
\end{lemma}

The next lemma asserts there will eventually be a uniform value for $root$. See Appendix \ref{A:UniformK-Value}.
\begin{lemma}
    %\label{L:UniformK-Value}
    Let $\mathcal{C}$ be an execution of the Self-Stabilizing Population Protocol. There exists a configuration $C \in \mathcal{C}$ appearing infinitely often such that all agents have the same index $\mathrm{root}$ in their agent states.
\end{lemma}

Letting $A$ be the input multiset to the population and $R$ be the root corresponding to $root$, we aim to show that if $root$ is such that $f(R) \neq f(A)$, then there is also an infinitely occurring configuration with uniform value of $root + 1$ for the index instead. Consequently, cycling through roots leads to an infinitely occurring configuration with $root$ such that $f(R)$ is the correct output for the given input.

If $f(R) \neq f(A)$, then $R \not \subseteq A$. Then there exists some other root $Right \in \mathcal{R}$ such that $Right \subseteq A$, implying $f(Right) = f(A)$ (and so $f(R) \neq f(Right)$). There are at least as many agents with input symbol $\sigma$ as there are occurrences of $\sigma$ in $Right$ (i.e. $m_A(\sigma) \geq m_{Right}(\sigma)$) since $Right$ is a \textit{subset} of the population's input. Thus the population would reject and increment $root$. The following lemma and corollary uses this reasoning to show that any population with uniform $root$ where $f(R) \neq f(A)$ will cycle through the root set until $root$ is incremented so that $f(R) = f(A)$. The proof is in Appendix \ref{A:InfiniteCorrectOutput}.
\begin{lemma}
    \label{L:InfiniteCorrectOutput}
    Let $\mathcal{C}$ be an execution of the Self-Stabilizing Population Protocol, let $R$ be the root corresponding to $\mathrm{root}$, and let the input to the population be $A$. There exists an infinitely occurring configuration $C \in \mathcal{C}$ such that all agents have the same $\mathrm{root}$ and $f(R) = f(A)$.
\end{lemma}
\begin{corollary}
    \label{C:CycleProperty}
    Let $\mathcal{C}$ be an execution of the Self-Stabilizing Population Protocol. If $C \in \mathcal{C}$ is an infinitely occurring configuration where all agents have the same $\mathrm{root}$ where $f(R) \neq f(A)$, then $C'$ is an infinitely occurring configuration in $\mathcal{C}$ where all agents have the same incremented index value of $\mathrm{root} + 1$.
\end{corollary}

Now certainly we cannot converge to an incorrect answer since an incorrect answer would lead us to a new value for $root$. To prove we do converge (to the right answer), we assume the protocol is not convergent. Then the population will keep cycling through indices of $root$ until we reach the corresponding root $Right \in \mathcal{R}$ such that $Right \subseteq A$. There cannot, then, be any other root $Wrong$ satisfying our condition $(*)$ to increment our $root$. If there was, then any $\sigma \in \Sigma$ where $m_{Wrong}(\sigma) > m_{Right}(\sigma)$ (occurrences of $\sigma$ happening strictly more in $Wrong$ than in $Right$) implies that there are at least $m_{Wrong}(\sigma)$ agents in the population (there are at least as many agents with $\sigma$ in the population as there are occurrences in $Wrong$). For all other $\sigma$ where $m_{Wrong}(\sigma) \leq m_{Right}(\sigma)$, we already know $Right \subseteq A$ and so $m_{Wrong}(\sigma) \leq m_A(\sigma)$; hence there are at least $m_{Wrong}(\sigma)$ agents in the population. Thus for all $\sigma \in \Sigma$ there are at least $m_{Wrong}(\sigma)$ agents in the population, meaning $Wrong \subseteq A \implies f(Wrong) = f(A)$. But $f(A) = f(Right) \neq f(Wrong)$, a contradiction. Thus the protocol must converge to the correct answer. The formal proof using this reasoning is left to Appendix \ref{A:SS-PP}.

\fi 

Sometimes it is interesting to create protocols that work on large classes of graphs (for instance, a protocol that decides whether the interaction graph has a vertex of degree greater than or equal to $k$ \cite{Aspnes}). When allowing the interaction graph $G$ to take on any form, we take the input as a mapping specifying which agents receive which inputs; since the output may change depending on the structure of the graph (like if it has a degree $\geq k$ vertex or not), we also include the interaction graph as input to the function. More formally, let $\mathcal{G}$ be a set of interaction graphs, and for any fixed graph $G = (V,E)$ let $A_G$ be a set of mappings $\alpha : V \rightarrow \Sigma$ for $G$. Define
\begin{gather*}
    \mathcal{Z}_\mathcal{G} = \{ (\alpha, G) \mid G \in \mathcal{G} \land \alpha \in A_G \}.
\end{gather*}
We then more generally define a larger class of population protocol functions.

\begin{definition}{\textit{Population Protocol Functions.}}
    Let $\mathcal{G}$ be a set of interaction graphs and $f: \mathcal{Z}_\mathcal{G} \rightarrow Y$ be a function. A population protocol $\mathcal{P}$ computes $f$ if and only if for any $(\alpha, G) \in \mathcal{Z}_\mathcal{G}$, $\mathcal{P}$ with input mapping $\alpha$ on interaction graph $G$ converges to $f((\alpha,G))$.
\end{definition}


\begin{aside}
    \textbf{Example}: Suppose our alphabet is $\Sigma = \{a, b\}.$ Let $\mathcal{X}$ be over this alphabet like so:
    \begin{align*}
        \mathcal{X} &= \{ \{ a, a, b, b\} \} \\
                    &\cup \{ \{a, b^3\}, \{a, b^4\}, \hdots \} \\
                    &\cup \{ \{b, a^3\}, \{b, a^4\}, \hdots \} \\
                    &\cup \{ \{a^3,b^3\}, \{ a^4, b^4 \}, \hdots \}.
    \end{align*}
    Suppose we had fixed $X = \{a, a, b, b\}$. Then $\mathcal{R}'_X = \{ \{a, a, b, b\} \}$ since there are no other multisets where \textbf{all} elements have multiplicity less than or equal to the respective multiplicity in $X$. The set $\mathcal{X} - \mbox{super}(\mathcal{R}'_X)$ is now just
    \begin{align*}
        \mathcal{X} - \mbox{super}(\mathcal{R}'_X) = \{ \{a, b^3\}, \{a, b^4\}, \hdots \} \cup \{ \{b, a^3\}, \{b, a^4\}, \hdots \}.
    \end{align*}
    For any $Y \in \mathcal{X} - \mbox{super}(\mathcal{R}'_X)$, it must be the case that 
    \begin{align*}
        m_Y(a) >  m_X(a) = 2 \iff m_Y(b) \leq m_X(b) = 2.
    \end{align*}
    Thus we know that \textit{exactly one} of the following cases it true:
    
    \begin{enumerate}
        \item $m_Y(a) = 0$ 
        \item $m_Y(a) = 1$ 
        \item $m_Y(a) = 2$ 
        \item $m_Y(b) = 0$ 
        \item $m_Y(b) = 1$
        \item $m_Y(b) = 2$ 
    \end{enumerate}
    There are no multisets in $\mathcal{X} - \mbox{super}(\mathcal{R}'_X)$ satisfying conditions (1), (3), (4), or (6); thus there will only be two sets in the partition: one with $a$ fixed with multiplicity 1 and one with $b$ fixed with mulitplicity 1.
    \begin{align*}
        \mathcal{X}_1 = \{ \{a, b^i\} \mid i \geq 3 \}, \\
        \mathcal{X}_2 = \{ \{b, a^i\} \mid i \geq 3 \}.
    \end{align*}
    
    The observation that follows is that we can remove $a$ from every multiset in $\mathcal{X}_1$ to generate a set of multisets over an alphabet of smaller size, which will have a root set by the inductive hypothesis; clearly adding $a$ back to every multiset of this root set will create a root set for $\mathcal{X}_1$.
\end{aside}







Since this is a construction on a model strictly weaker than the more general globally-fair scheduled systems specified earlier, this also implies the converse of Theorem \ref{Turing Machine Self-Stabilization} when interaction graphs are complete.


\begin{corollary}[Globally Fair Self-Stabilization Theorem]
    Let $f: \mathcal{X} \rightarrow \{0,1\}$ be a function computable by a globally-fair scheduled system, where without loss of generality we take $\mathcal{X}$ as a set of multisets. Then
    \begin{align*}
        f \text{ has a self-stabilizing solution} \iff (\forall A,B \in \mathcal{X}, A \subseteq B \implies f(A) = f(B)).
    \end{align*}
\end{corollary}
\begin{proof}
    The forward implication is an implication of Theorem \ref{Turing Machine Self-Stabilization}. The right hand side implies a self-stabilizing population protocol for $f$ by the Self-Stabilizing Population Protocol Theorem. A globally-fair scheduled system can emulate a population protocol by having each agent be a finite state machine and have interactions between two agents result in the sharing of each other's states and then a consequent transition for each agent. Thus the system could emulate the self-stabilizing population protocol, and would inherit that self-stabilizing property.
\end{proof}    
    
    
    
    
    
    

We can in fact make a more general statement about self-stabilizing protocols designed to work on various different interaction graphs, using the same proof, which can be viewed in the Appendix.

\begin{theorem}
    Let $\mathcal{P} = (Q, \Sigma, Y, I, O, \delta)$ be a self-stabilizing population protocol computing some function $f: \mathcal{Z}_\mathcal{G} \rightarrow Y$. Let $(\alpha, G=(V,E)),(\alpha', G'=(V',E')) \in \mathcal{Z}_\mathcal{G}$ be such that $G$ is isomorphic to a subgraph of $G'$ via bijection $\beta: V \rightarrow V'$. Then
    \begin{gather*}
        \left (\forall v \in V, \alpha(v) = \alpha'(\beta(v)) \right ) \implies f((\alpha, G)) = f((\alpha', G')).
    \end{gather*}
\end{theorem}


Note that Theorem 4.2 is a stronger statement than Theorem 4.1, since the latter is a corollary (it is a specific case of the former). This is evident when we restrict our graphs to only complete interaction graphs, in which any graph with fewer vertices than another will naturally be a subgraph. Massaging the input mappings back into the normal multiset form (which can be done since agents are indistinguishable if the interaction graph is complete) will yield the first theorem for the basic model.

Furthermore, it is interesting to note that these proofs \textit{never} invoke the fact that the agents are finite state machines. In fact if we were to replace the finite state machines with, say, Turing Machines under similar scheduling constraints, the argument is identical. Moreover, the following section will demonstrate that the necessary conditions shown here are actually sufficient in population protocols, and thus would be sufficient for any other stronger models. Therefore this characterization for population protocols holds for any analogous system with a globally-fair scheduler.

\begin{theorem}\label{Turing Machine Self-Stabilization}
    Let $f: \mathcal{Z}_\mathcal{G} \rightarrow Y$ be a function computed by a globally fair scheduled system via some distributed algorithm $\mathcal{A}$ on a family of interaction graphs $\mathcal{G}$. Let $(\alpha, G),(\alpha', G') \in \mathcal{Z}_\mathcal{G}$ be such that $G = (V, E)$ is isomorphic to a subgraph of $G' = (V',E')$ via bijection $\beta: V \rightarrow V'$. Then
    \begin{gather*}
        \left ( \forall v \in V, \alpha(v) = \alpha'(\beta(v)) \right ) \implies f((\alpha, G)) = f((\alpha', G')).
    \end{gather*}
\end{theorem}
\begin{proof}
    Suppose that we have $(\alpha, G=(V,E)),(\alpha', G'=(V',E')) \in \mathcal{Z}_\mathcal{G}$ such that the conditions above hold, and yet $f((\alpha,G)) \neq f((\alpha', G'))$. Let $\mathcal{A}$ run on graph $G'$ with input mapping $\alpha'$; by correctness of $\mathcal{A}$, every member of the population will eventually output $f((\alpha', G'))$ for all time. By global fairness the scheduler can act arbitrarily for a finite amount of time, and so we can schedule interactions only amongst the subgraph of $G'$ that $G$ is isomorphic to. Since all the agents in the isomorphic graph have the same input mapping as determined by $\alpha$, we are effectively running $\mathcal{A}$ on $G$ with input mapping $\alpha$ from some arbitrary configuration. Since $\mathcal{A}$ is self-stabilizing, after a finite number of steps all agents in the subgraph should be outputting $f((\alpha,G))$. However this contradicts the convergence of the general population since $f((\alpha,G)) \neq f((\alpha', G'))$. Hence it must be that $f((\alpha,G)) = f((\alpha', G'))$.
\end{proof}


\section{Proof of Theorem 4.2}
\begin{theorem*}
    Let $\mathcal{P} = (Q, \Sigma, Y, I, O, \delta)$ be a self-stabilizing population protocol computing some function $f: \mathcal{Z}_\mathcal{G} \rightarrow Y$. Let $(\alpha, G=(V,E)),(\alpha', G'=(V',E')) \in \mathcal{Z}_\mathcal{G}$ be such that $G$ is isomorphic to a subgraph of $G'$ via bijection $\beta: V \rightarrow V'$. Then
    \begin{gather*}
        \left (\forall v \in V, \alpha(v) = \alpha'(\beta(v)) \right ) \implies f((\alpha, G)) = f((\alpha', G')).
    \end{gather*}
\end{theorem*}
\begin{proof}
    Suppose that we have $(\alpha, G=(V,E)),(\alpha', G'=(V',E')) \in \mathcal{Z}_\mathcal{G}$ such that the conditions above hold, and yet $f((\alpha,G)) \neq f((\alpha', G'))$. Allow protocol $\mathcal{P}$ to run on graph $G'$ with input mapping $\alpha'$; by correctness of the protocol, it should eventually converge to $f((\alpha',G'))$. Let $H$ be the subgraph of $G'$ that $G$ is isomorphic to via bijection $\beta$. By global fairness we can have the scheduler act arbitrarily for a finite number of steps; therefore we can have the scheduler only schedule interactions amongst agents in subgraph $H$ for a finite amount of steps. Since by our hypothesis all agents in $G$ have the same inputs as their analogous agents in $H$, we can view the running of the protocol on subgraph $H$ as a finitely long execution of $\mathcal{P}$ on graph $G$ with input mapping $\alpha$. Such an execution must eventually converge to $f((\alpha,G))$ after some finitely many steps since the protocol is self-stabilizing, and thus agents in subgraph $H$ will eventually output $f((\alpha,G))$. However this contradicts convergence, since $f((\alpha,G)) \neq f((\alpha', G'))$. Therefore no such inputs can exist, and the theorem holds.
\end{proof}


As a toy example, fix a function $f: \mathcal{X} \rightarrow Y$ (with the property that $A \subseteq B \implies f(A) = f(B)$). Further suppose that $$\mathcal{R} = \{ \{a, a, a, b\}, \{b, b, b, a\} \}$$ is a root set of $\mathcal{X}$, where $f(\{a, a, a, b\}) = 1$ and $f(\{b, b, b, a\}) = 0$. Let the agent states be:

\begin{center}
\begin{tabular}{ccccc}
    $(q_a^0, 0)$ & $(q_a^0, 1)$ & $(q_a^1, 0)$ & $(q_a^1, 1)$ & $(q_a^2, 0)$ & $(q_a^2, 1)$ \\
    $(q_b^0, 0)$ & $(q_b^0, 1)$ & $(q_b^1, 0)$ & $(q_b^1, 1)$ & $(q_b^2, 0)$ & $(q_b^2, 1)$ \\
\end{tabular}
\end{center}

The transitions are as follows.

\begin{center}
\begin{tabular}{|c|c|c|c|}
    \hline
    Initiator Initial (State, Input) & Responder Initial (State, Input) & Initiator Transition State & Responder Transition State \\
    \hline 
    
    \hline
    $((q_i^j, u),i)$ & $((q_i^j, v),i)$ & $(q_i^j, u)$ & $(q_i^{j + 1 \mod 3}, v)$ \\
    \hline
    $((x,0), i)$ & $((y, 1), j)$ & $(x, 0)$ & $(y, 0)$ \\
    \hline
    $((x,1),i)$ & $((y, 0),j)$ & $(x, 1)$ & $(y, 1)$ \\
    \hline
    $((q_a^2, u),a)$ & $((y, v),j)$ & $(q_a^0, 1)$ & $(y, 1)$ \\
    \hline
    $((q_b^2, u),b)$ & $((y, v),j)$ & $(q_b^0, 0)$ & $(y, 0)$ \\
    \hline
\end{tabular}
\end{center}

If the input is a superset of $\{b, b, b, a\}$, there are at least 3 agents with input $b$. Suppose we do not converge to $f(\{b, b, b, a\}) = 0$. Then there must be some infinitely occurring configuration $C$ where at least one agent is outputting 1. Have this agent initiate an interaction with each other agent; by the third row of the table all agents will now be outputting 1. If none of the agents have state $q_b^2$ then since there are at least three agents two of them have the same state $q_b^0$ or $q_b^1$; having duplicates interact causes the superscript to increment, so eventually there will be an agent with state $q_b^2$. Let $C'$ be the configuration $C \rightarrow C'$ following configuration $C$ such that the agent with $(q_b^2, 0)$ initiates an interaction with everyone. This will force everyone to switch to 0. Since $C$ is infinitely occurring and $C \rightarrow C'$, by global fairness $C'$ is infinitely occurring. The same argument works analogously if the input is a superset of $\{a, a, a, b\}$.

This example generally follows the principles outlined in the beginning of this section: for whichever root 

\begin{table}[H]
        \centering
        \hspace*{-4cm}
        \begin{tabular}{|c|c|cc|}
            \hline
            Initiator & Responder & Output of $\delta$ & \\
            \hline
            
            & \multirow{4}{*}{$((*, *, *, \hdots, *),*)$} & \multirow{3}{*}{$((q_a^0, *, *, \hdots, *), (*, *, *, \hdots, *))$} & \multirow{4}{*}{(2a)}\\
            $((q_i^j, *, *, \hdots, *), a)$ & & & \\
            where $i \neq a$ & & & \\
            & & & \\
            \hline
            
            \multirow{5}{*}{$((q_a^j, k, *, \hdots, *), a)$} & & \multirow{5}{*}{$((q_a^0, k', \vec{r}_1, \hdots, \vec{r}_{|\mathcal{R}|}), (q_b^{j'}, k', \vec{r}_1, \hdots, \vec{r}_{|\mathcal{R}|}))$} & \multirow{5}{*}{(2b)}\\
            & $((q_{b}^{j'}, k', \vec{r}_1, \hdots, \vec{r}_{|\mathcal{R}|}), b)$ & &\\
            & where $k' > k$ & & \\
            & and $(k' \neq |\mathcal{R}| - 1$ or $k \neq 0)$ & & \\
            & & & \\
            \hline
            
            \multirow{3}{*}{$((q_a^j, |\mathcal{R}| - 1, *, \hdots, *), a)$} & \multirow{3}{*}{$((q_{b}^{j'}, 0, \vec{r}_1, \hdots, \vec{r}_{|\mathcal{R}|}), b)$} & \multirow{3}{*}{$((q_a^0, |\mathcal{R}| - 1, \vec{r}_1, \hdots, \vec{r}_{|\mathcal{R}|}), (q_b^{j'}, |\mathcal{R}| - 1, \vec{r}_1, \hdots, \vec{r}_{|\mathcal{R}|}))$} & \multirow{3}{*}{(2c)} \\
            & & & \\ 
            & & & \\
            \hline
            
            \multirow{3}{*}{$((q_a^j, 0, *, \hdots, *), a)$} & \multirow{3}{*}{$((q_{b}^{j'}, |\mathcal{R}| - 1, \vec{r}_1, \hdots, \vec{r}_{|\mathcal{R}|}), b)$} & \multirow{3}{*}{$((q_a^0, 0, \vec{r}_1, \hdots, \vec{r}_{|\mathcal{R}|}), (q_b^{j'}, 0, \vec{r}_1, \hdots, \vec{r}_{|\mathcal{R}|}))$} & \multirow{3}{*}{(2d)} \\
            & & & \\ 
            & & & \\
            \hline
            
            & & & \\
            \multirow{8}{*}{$((q_a^j, k, \vec{r}_1, \hdots, \vec{r}_{|\mathcal{R}|}),a)$} & & $((q_a^0, k + 1, \vec{0}, \hdots, \vec{0}), (q_b^0, k + 1, \vec{0}, \hdots, \vec{0}))$ & \multirow{8}{*}{(2e)}\\ 
            & & if $\exists n, \vec{r}_n \lor \vec{s}_n = 1^{|A_{n,k}|}$ & \\
            & & Addition taken modulo $|\mathcal{R}|$ & \\
            & $((q_{b}^{j'}, k, \vec{s}_1, \hdots, \vec{s}_{|\mathcal{R}|}),b)$ & & \\
            \cdashline{3-3}
            & where $j \neq j'$ & & \\ 
            & & $((q_a^j, k, \vec{r}_1 \lor \vec{s}_1, \hdots, \vec{r}_{|\mathcal{R}|} \lor \vec{s}_{|\mathcal{R}|}),(q_b^{j'}, k, \vec{s}_1 \lor \vec{r}_1, \hdots, \vec{s}_{|\mathcal{R}|} \lor \vec{r}_{|\mathcal{R}|}))$ & \\
            & & o.w. & \\
            & & & \\
            \hline
            
            \multirow{4}{*}{$((q_a^j, k, *, \hdots, *),a)$} & \multirow{4}{*}{$((q_a^j, k, *, \hdots, *), a)$} & & \multirow{4}{*}{(2f)} \\
            & & $((q_a^j, k, *, \hdots, *), (q_a^{j+1}, k, *, \hdots, *))$ & \\
            & & Addition taken modulo $\left ( \max_{R \in \mathcal{R}} m_R(i)  \right )$ & \\
            & & & \\
            \hline
        \end{tabular}
        \hspace*{-3cm}
        \caption{Self-Stabilizing Population Protocol transitions. We take $*$ as a wildcard character and $\vec{r} \lor \vec{s}$ as a bitwise OR. $(2a)$  $(2b)$  $(2c)$ and $(2d)$ say that if those values are both 0 and $|\mathcal{R}| - 1$ then both agents resolve to the initiator's $k$-value.  $(2e)$  Finally $(2f)$ .}
    \end{table}
